Diverse Imagenet Models Transfer Better

A commonly accepted hypothesis is that models with higher accuracy on Imagenet perform better on other downstream tasks, leading to much research dedicated to optimizing Imagenet accuracy. Recently this hypothesis has been challenged by evidence showing that self-supervised models transfer better than their supervised counterparts, despite their inferior Imagenet accuracy. This calls for identifying the additional factors, on top of Imagenet accuracy, that make models transferable. In this work we show that high diversity of the features learnt by the model promotes transferability jointly with Imagenet accuracy. Encouraged by the recent transferability results of self-supervised models, we propose a method that combines self-supervised and supervised pretraining to generate models with both high diversity and high accuracy, and as a result high transferability. We demonstrate our results on several architectures and multiple downstream tasks, including both single-label and multi-label classification.

==> abstract_v1.tex <==
\begin{abstract}
A hypothesis in modern computer vision research is that models that perform better on ImageNet necessarily perform better on other vision tasks.
% Models that preform well on Imagenet are believed to transfer better to downstream tasks. 
However, self-supervised Imagenet models are shown to transfer even better than their supervised counterparts, despite their inferior Imagenet accuracy. This calls for identifying the missing factors, apart from Imagenet performance, that make models transferable and to combine both self-supervised and supervised pretrainig for generating more transferable models. We show that besides Imagenet performance, the diversity of features learnt by the model promotes transferability and thus we propose a simple method to control the supervision applied to self-supervised models for maintaining high diversity and generating more transferable models. We demonstrate our results over 15 different single-label image classification downstream datasets and a multi-label classification downstream task. 
\keywords{Transfer Learning, Self-Supervised Learning, Supervised Learning}
\end{abstract}

==> experiments/multi_label_res.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|c|c}
\toprule
           Pretrain &  ImNet &  COCO \\
\toprule
 Vanilla CE &  78.70 &          81.95 \\ 
  SupCon~\cite{khosla2020supervised} & 77.35 & 81.29 \\
 \hline
   CE+SelfSupCon & 77.33 &  82.05 \\
   MoCo-v2 &  61.89 &          78.70  \\
   MoCo-v2 ($\mathcal{T}=1$) &  78.73 &          81.94 \\
    MoCo-v2 ($\mathcal{T}=4$) &  76.04 &          81.74 \\
    \hline
   SwAV &  64.20 &          82.86 \\
    SwAV ($\mathcal{T}=1$) &  79.17 &          82.38 \\
     SwAV ($\mathcal{T}=4$) &  78.08 &          \textbf{83.28} \\
     \hline
   DINO &  74.98 &   82.74       \\
   DINO ($\mathcal{T}=1$)& 77.62  &   82.33        \\
   DINO ($\mathcal{T}=4$)& 77.46 &    83.10        \\
     \hline
   SimCLR &   68.09 &   80.51       \\
   SimCLR ($\mathcal{T}=1$)&  78.07  &   81.29        \\
   SimCLR ($\mathcal{T}=4$)& 74.95  &   81.51     \\
\bottomrule
\end{tabular}
\caption{Performance of different models fine-tuned on  MS-COCO multi-label classification dataset in terms of mAP (\%). Label injected models transfer best.}
\label{tab:cnn_multilabel}
\end{table}


==> experiments/multi_label_res_full.tex <==
\begin{tabular}{lrr}
\toprule
           Pretrain &  ImNet &  TL\_multilabel \\
\midrule
 resnet50\_200\_epoch &  78.70 &          81.95 \\
 resnet50\_600\_epoch &  79.40 &          82.01 \\
      base\_finetune &  76.38 &          81.79 \\
     base\_plus\_moco &  77.33 &          82.02 \\
   moco2\_ft\_1\_98615 &  78.73 &          81.96 \\
   moco2\_ft\_2\_98614 &  77.67 &          81.89 \\
   moco2\_ft\_3\_98613 &  77.01 &          81.78 \\
   moco2\_ft\_4\_98612 &  76.04 &          81.74 \\
   moco2\_ft\_5\_98611 &  75.67 &          81.65 \\
  moco2\_ft\_10\_98610 &  73.25 &          81.19 \\
  moco2\_ft\_50\_98609 &  66.20 &          80.11 \\
 moco2\_ft\_100\_98608 &  62.56 &          79.71 \\
              moco2 &  61.89 &          78.67 \\
    swav\_ft\_1\_80999 &  79.17 &          82.38 \\
    swav\_ft\_2\_86226 &  78.96 &          82.60 \\
    swav\_ft\_3\_85901 &  78.59 &          83.02 \\
    swav\_ft\_4\_86225 &  78.08 &          83.28 \\
    swav\_ft\_5\_85308 &  77.58 &          83.28 \\
   swav\_ft\_10\_85314 &  76.13 &          83.21 \\
   swav\_ft\_50\_85315 &  73.20 &          82.94 \\
  swav\_ft\_100\_85316 &  72.00 &          82.91 \\
               swav &  64.20 &          82.86 \\
\bottomrule
\end{tabular}

==> experiments/single_label_res_full_linprob.tex <==
\begin{table}[htb]
\centering
\tiny
\begin{tabular}{l|c|ccccccccccc|c}
\toprule
Pretrain &  
\rotatebox[origin=c]{-70}{ImNet} &  
\rotatebox[origin=c]{-70}{Flowers} &  
\rotatebox[origin=c]{-70}{Caltech} &  
\rotatebox[origin=c]{-70}{CIFAR10}&  
\rotatebox[origin=c]{-70}{CIFAR100}&  
\rotatebox[origin=c]{-70}{DTD}&  
\rotatebox[origin=c]{-70}{Aircraft} &  
\rotatebox[origin=c]{-70}{Food}&  
\rotatebox[origin=c]{-70}{Birds}&  
\rotatebox[origin=c]{-70}{Cars}&  
\rotatebox[origin=c]{-70}{Dogs}&  
\rotatebox[origin=c]{-70}{Sun}&  
\rotatebox[origin=c]{-70}{Transfer}\\
\midrule
Supervised &           78.7 &     86.5 &         89.0 &     92.8 &      77.1 & 69.6 &           42.1 &     70.0 &     60.7 &           59.3 &           90.4 &    63.1 &      15.7 \\
Supervised (Long) &           79.4 &     86.9 &         89.0 &     93.2 &      76.8 & 70.8 &           43.1 &     69.8 &     61.2 &           59.5 &           91.6 &    63.9 &      19.2 \\
SupCon                      &            NaN &     89.0 &         85.9 &     90.9 &      68.9 & 55.4 &           45.2 &     54.5 &     37.8 &           65.5 &           85.9 &    40.7 &       NaN \\
\midrule
DINO ($\mathcal{T} = 1$)         &           77.6 &     86.9 &         89.1 &     93.3 &      78.0 & 69.8 &           39.9 &     70.5 &     62.8 &           57.8 &           91.0 &    64.2 &      18.1 \\
DINO ($\mathcal{T} = 2$)         &           77.7 &     89.4 &         89.0 &     93.4 &      78.1 & 71.5 &           44.2 &     72.4 &     64.3 &           59.7 &           89.3 &    65.3 &      23.6 \\
DINO ($\mathcal{T} = 3$)         &           77.6 &     90.8 &         89.7 &     93.8 &      78.8 & 71.1 &           45.5 &     73.4 &     65.4 &           60.3 &           88.1 &    65.9 &      27.1 \\
DINO ($\mathcal{T} = 4$)         &           77.5 &     91.8 &         89.5 &     93.6 &      79.0 & 71.3 &           47.6 &     74.0 &     65.4 &           60.9 &           86.8 &    65.8 &      28.3 \\
DINO ($\mathcal{T} = 5$)         &           77.1 &     91.7 &         89.1 &     93.4 &      79.1 & 71.3 &           48.0 &     74.5 &     65.4 &           61.7 &           85.7 &    65.6 &      27.4 \\
DINO ($\mathcal{T} = 10$)        &           76.5 &     92.2 &         88.6 &     93.2 &      79.1 & 70.6 &           49.7 &     74.0 &     64.7 &           64.3 &           83.0 &    65.0 &      25.9 \\
DINO ($\mathcal{T} = 50$)        &           76.1 &     92.5 &         87.7 &     92.9 &      78.1 & 68.6 &           51.2 &     73.1 &     62.2 &           64.8 &           77.4 &    62.9 &      18.8 \\
DINO ($\mathcal{T} = 100$)       &           75.8 &     92.7 &         87.7 &     93.0 &      77.8 & 67.4 &           50.3 &     72.3 &     60.3 &           65.7 &           75.4 &    62.0 &      16.1 \\
DINO                          &           75.0 &     92.6 &         86.1 &     90.9 &      71.3 & 64.6 &           48.6 &     68.8 &     47.6 &           66.8 &           65.9 &    56.1 &      -4.8 \\
\midrule
SimCLR ($\mathcal{T} = 1$)       &           78.1 &     87.6 &         88.7 &     93.8 &      77.6 & 70.2 &           43.0 &     70.3 &     60.8 &           57.8 &           88.8 &    64.0 &      17.0 \\
SimCLR ($\mathcal{T} = 2$)       &           77.1 &     87.4 &         88.1 &     93.6 &      77.6 & 68.8 &           45.4 &     70.1 &     58.3 &           56.4 &           86.5 &    63.9 &      12.9 \\
SimCLR ($\mathcal{T} = 3$)       &           75.8 &     87.6 &         87.9 &     93.5 &      77.8 & 68.5 &           43.7 &     69.6 &     56.6 &           57.3 &           84.3 &    63.1 &       9.4 \\
SimCLR ($\mathcal{T} = 4$)       &           75.0 &     87.8 &         87.5 &     93.5 &      77.6 & 68.5 &           45.2 &     68.8 &     54.9 &           56.7 &           82.5 &    62.8 &       7.2 \\
SimCLR ($\mathcal{T} = 5$)       &           74.3 &     88.2 &         87.3 &     93.0 &      76.9 & 67.9 &           45.9 &     68.5 &     53.6 &           56.8 &           81.2 &    62.6 &       5.1 \\
SimCLR ($\mathcal{T} = 10$)      &           73.1 &     87.7 &         86.5 &     92.9 &      76.9 & 66.4 &           43.4 &     67.5 &     50.7 &           56.3 &           77.6 &    61.2 &      -1.9 \\
SimCLR ($\mathcal{T} = 50$)      &           69.9 &     86.9 &         84.2 &     92.1 &      72.7 & 61.5 &           39.3 &     61.8 &     37.9 &           50.9 &           66.1 &    56.3 &     -26.9 \\
SimCLR ($\mathcal{T} = 100$)     &           69.4 &     86.5 &         83.6 &     91.6 &      71.6 & 60.9 &           36.8 &     61.2 &     36.5 &           50.4 &           64.7 &    55.4 &     -31.8 \\
SimCLR                        &           68.1 &     85.0 &         82.4 &     87.8 &      63.9 & 60.3 &           36.7 &     58.9 &     33.9 &           47.1 &           61.2 &    52.8 &     -46.5 \\
\midrule
% base\_finetune                 &           76.4 &     78.6 &         83.4 &     90.6 &      71.4 & 62.1 &           26.4 &     60.4 &     52.5 &           39.7 &           96.6 &    56.7 &     -15.2 \\
CE + SelfSupCon      &           77.3 &     85.6 &         87.1 &     93.0 &      76.0 & 65.6 &           34.2 &     65.1 &     52.3 &           50.1 &           93.9 &    61.3 &       3.7 \\
MoCo-v2 ($\mathcal{T} = 1$)        &           78.7 &     80.0 &         86.7 &     92.3 &      74.4 & 66.8 &           29.9 &     64.5 &     55.2 &           45.9 &           91.6 &    60.6 &      -7.4 \\
MoCo-v2 ($\mathcal{T} = 2$)        &           77.7 &     80.7 &         87.0 &     92.2 &      74.3 & 66.4 &           32.8 &     64.4 &     56.0 &           47.1 &           89.7 &    60.5 &      -7.3 \\
MoCo-v2 ($\mathcal{T} = 3$)        &           77.0 &     82.0 &         86.5 &     92.1 &      74.7 & 65.5 &           34.1 &     64.8 &     57.0 &           47.8 &           88.2 &    59.9 &      -7.6 \\
MoCo-v2 ($\mathcal{T} = 4$)        &           76.0 &     82.7 &         86.4 &     92.0 &      74.1 & 64.9 &           35.1 &     64.8 &     56.8 &           49.3 &           87.4 &    60.4 &      -7.4 \\
MoCo-v2 ($\mathcal{T} = 5$)        &           75.7 &     83.3 &         86.6 &     91.4 &      74.4 & 64.8 &           36.2 &     64.5 &     56.6 &           47.2 &           86.2 &    59.3 &      -9.3 \\
MoCo-v2 ($\mathcal{T} = 10$)       &           73.2 &     83.3 &         85.3 &     91.5 &      73.3 & 64.7 &           37.3 &     62.8 &     55.1 &           48.7 &           83.6 &    58.4 &     -13.1 \\
MoCo-v2 ($\mathcal{T} = 50$)       &           66.2 &     81.6 &         82.2 &     90.0 &      69.8 & 60.5 &           34.7 &     57.9 &     49.2 &           45.7 &           75.7 &    53.3 &     -33.7 \\
MoCo-v2 ($\mathcal{T} = 100$)      &           62.6 &     81.0 &         81.6 &     88.8 &      67.8 & 57.4 &           34.0 &     55.3 &     45.2 &           44.0 &           71.4 &    50.0 &     -44.2 \\
MoCo-v2                         &           61.9 &     84.5 &         58.8 &     81.5 &      45.2 & 53.2 &           34.8 &     31.2 &     10.1 &           47.7 &           37.1 &    30.4 &    -113.8 \\
% supervised\_mean2              &            NaN &     90.6 &         85.8 &     91.2 &      67.8 & 56.1 &           45.8 &     56.9 &     34.5 &           65.4 &           83.2 &    43.0 &       NaN \\
\midrule
SwAV ($\mathcal{T} = 1$)         &           79.2 &     86.5 &         88.9 &     93.2 &      77.0 & 69.8 &           39.1 &     69.6 &     62.3 &           54.4 &           91.1 &    63.5 &      14.7 \\
SwAV ($\mathcal{T} = 2$)         &           79.0 &     88.5 &         88.9 &     93.4 &      78.1 & 70.5 &           42.5 &     70.8 &     63.6 &           56.6 &           89.8 &    64.8 &      19.7 \\
SwAV ($\mathcal{T} = 3$)         &           78.6 &     89.5 &         89.5 &     92.9 &      77.9 & 70.3 &           44.4 &     72.0 &     64.4 &           58.9 &           88.4 &    65.7 &      21.8 \\
SwAV ($\mathcal{T} = 4$)         &           78.1 &     90.2 &         89.6 &     93.0 &      78.6 & 70.6 &           48.0 &     72.2 &     65.1 &           58.9 &           87.1 &    65.5 &      23.8 \\
SwAV ($\mathcal{T} = 5$)         &           77.6 &     90.2 &         89.1 &     93.3 &      78.5 & 70.7 &           47.0 &     72.6 &     64.7 &           59.4 &           85.8 &    65.4 &      22.3 \\
SwAV ($\mathcal{T} = 10$)        &           76.1 &     90.7 &         88.7 &     93.2 &      78.5 & 69.9 &           47.4 &     72.6 &     64.3 &           61.5 &           83.3 &    64.5 &      20.9 \\
SwAV ($\mathcal{T} = 50$)        &           73.2 &     91.3 &         88.0 &     92.7 &      77.7 & 67.5 &           50.6 &     71.4 &     61.6 &           62.9 &           78.3 &    62.4 &      15.1 \\
SwAV ($\mathcal{T} = 100$)       &           72.0 &     91.1 &         87.8 &     92.5 &      76.7 & 66.6 &           50.2 &     70.7 &     59.5 &           65.1 &           76.4 &    61.3 &      11.6 \\
SwAV                          &           72.0 &     90.6 &         85.7 &     90.2 &      69.3 & 63.4 &           45.4 &     65.4 &     44.7 &           61.8 &           66.6 &    53.6 &     -15.8
\bottomrule
\end{tabular}
\caption{Linear probing performance of different \textbf{CNN} models, including different levels of label injected models) fine-tuned on the downstream datasets in terms of top-1 accuracy (\%) and the overall transferability score. The models are grouped by the underlying base SSL method.} 
\label{tab:full_table_linprob}
\end{table}

==> intro_asaf.tex <==
\section{Alternative Introduction (Asaf)}
The success of Deep Neural Networks (DNNS) in a variety of computer vision tasks is largely related to their ability to transfer feature representations learned on a pre-trained task to leverage others.
A common practice is to pre-train a model on a large-scale supervised dataset such as ImageNet~\cite{russakovsky2015imagenet} and fine-tune it on the downstream (target) dataset that is typically of a smaller scale.
This practice has systematically advanced the state-of-the-art in tasks such as image classification~\cite{liu2021query2label,ridnik2021ml}, object detection~\cite{liu2021swin,ren2015faster} and semantic segmentation~\cite{he2017mask,liu2021swin}.
The pursuit after better pretrained models coincided with pushing the state-of-the-art performance on ImageNet, as it was shown that supervised pre-trained models that perform better on ImageNet also tend to perform better when fine-tuned on other vision tasks \cite{kornblith2019better}.

Recent works demonstrate that self-supervised pre-training (SSL) without any label information can also learn effective representations from upstream data (e.g., ImageNet) and even surpass supervised methods when transferring to downstream tasks.
This success in transfer learning, despite their relatively poor performance on ImageNet \cite{chen2020simple,he2020momentum,grill2020bootstrap,chen2021exploring,zbontar2021barlow,ericsson2021well} calls for identifying the additional factors on top of Imagenet accuracy, that make models transferable.

----

a













While supervised training focuses on class-level discrimination, SSL focuses on instance discrimination, and models are trained to keep variants of the same instance close together in the representation space, and sometimes also, separated from different instances.
On the other hand, supervised models learn meaningfull high-level semantic features that are shared between instances of the same class, while SSL might capture irrelevant low level visual features (e.g., related to instance background). Thus high ImageNet performance guarantees that the features learnt are semantically meaningful and SSL learns diverse features.
This observation is supported by recent work that combines both supervised and self-supervised losses to improve transferability \cite{khosla2020supervised,islam2021broad}, yet those require intervention in the self-supervision stage and the transferability is attributed to other less important factors than feature diversity such as the abstraction of the representations learned (measured by Centered Kernel Alignment (CKA)~\cite{kornblith2019similarity} between layers) and intra-class variations.

Our contribution is two-fold: (1) We propose \textit{Feature Diversity} as a calibration for the Imagenet accuracy for assessing the transferability of pre-trained models.
\begin{align}
\textit{Calibrated Imagenet Score} = \text{Imagenet Accuracy} \times \text{Feature Diversity}
\end{align}
As we empirically validate that \textit{Calibrated Imagenet Score (CIS)} better correlates with trasferability, as shown in Figure~\ref{fig:tl_correlation_asaf}.

(2) We introduce a simple training method \textit{Controlled Label Injection (CLI)}, that enables the injection of label information into any self-supervised pre-trained model in a controlled manner, for generating models of different feature diversity and Imagenet accuracy. The resulted models increase ImageNet performance while either improving or maintaining feature diversity of the self-supervised model.
This both allows us to make observations about the connection between the CIS and transferability, while at the same time this leads to models with higher transferability.

We validate our approach over both CNNs (ResNets~\cite{he2016deep}) and vision transformers (ViT~\cite{dosovitskiy2021an}), several self-supervised pre-training methods (e.g., MoCo-v2~\cite{chen2020improved},
SimCLR~\cite{chen2020simple},
SwAV~\cite{caron2020unsupervised}, DINO~\cite{caron2020unsupervised} and MAE~\cite{MaskedAutoencoders2021}), two formulations of Feature Diversity, several downstream vision tasks, including multi-label classification on the MS-COCO~\cite{lin2014microsoft} dataset and a variety of 14 single-label classification datasets.

In section~\ref{sec:feature_diversity} we introduce the notion of feature diversity.  In section~\ref{sec:LabelInjection}, we describe the \textit{Controlled Label Injection} scheme, for generating models of different feature diversity and Imagenet accuracy.
In section~\ref{sec:exp}, we describe the experimental settings and show that the label injected models have higher transferability than alternative ways for combining SSL with superived models. In section~\ref{sec:fesature_importance}, we show that Feature Diversity is more important for transferability than other previously suggested factors~\cite{kornblith2021better,islam2021broad}, such as the level of abstraction learnt by the model and class separation.
% We measure the diversity of the learned features and empirically confirm that feature diversity plays an important role, together with ImagenNet performance, in the transferability of the pre-trained model.

\begin{figure}[htb]
\centering
\begin{subfigure}{.49\textwidth}
  \centering
    \includegraphics[width=0.98\textwidth, height=!]{figures/r2_imagenet.pdf}
  \label{fig:label_injection_cka}
\end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \centering
%     \includegraphics[width=0.98\textwidth, height=!]{figures/r2_spectral_calibrated_imagenet.pdf}
%   \label{fig:label_injection_calibrated}
% \end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
    \includegraphics[width=0.98\textwidth, height=!]{figures/r2_calibrated_imagenet.pdf}
  \label{fig:label_injection_calibrated}
\end{subfigure}

% \caption{Transferability vs Imagent accuracy (Left), the Spectral Feature Diversity based CIS (Middle) and the Clustering Feature Diversity based CIS. The Calibrated Imagenet Score correlates with transferability significantly better.}
\caption{Transferability vs Imagent accuracy (Left) and the Clustering Feature Diversity based CIS for 40 models pre-trained via supervised, self-supervised learning and their combinations. The Calibrated Imagenet Score correlates with transferability significantly better.}
\label{fig:tl_correlation_asaf}
\end{figure}

==> intro_avram.tex <==
\section{Introduction}
The success of Deep Neural Networks (DNNS) in a variety of computer vision tasks is largely related to their ability to transfer feature representations learned on a pre-trained task to leverage others.
A common practice is to pre-train a model on a large-scale supervised dataset such as ImageNet~\cite{russakovsky2015imagenet} and fine-tune it on the downstream (target) dataset that is typically of a smaller scale.
This practice has systematically advanced the state-of-the-art in tasks such as image classification~\cite{liu2021query2label,ridnik2021ml}, object detection~\cite{liu2021swin,ren2015faster} and semantic segmentation~\cite{he2017mask,liu2021swin}.
The pursuit after better pretrained models coincided with pushing the state-of-the-art performance on ImageNet, as it was shown that supervised pre-trained models that perform better on ImageNet also tend to perform better when fine-tuned on other vision tasks \cite{kornblith2019better}.

Recent works demonstrate that self-supervised pre-training (SSL) without any label information can also learn effective representations from upstream data (e.g., ImageNet) and even surpass supervised methods when transferring to downstream tasks.
This success in transfer learning, despite their relative poor performance on ImageNet \cite{chen2020simple,he2020momentum,grill2020bootstrap,chen2021exploring,zbontar2021barlow,ericsson2021well} calls for identifying the additional factors, on top of Imagenet accuracy, that make models transferable.

While supervised training focuses on class-level discrimination, SSL focuses on instance discrimination, and models are trained to keep variants of the same instance close together in the representation space, and sometimes also, separated from different instances.
Thus the self-supervised approach effectively captures richer and more diverse and discriminative features of varying levels of abstraction, that are useful for many downstream tasks, compared to more high level class-discriminative features learned by supervised methods.
On the other hand, supervised models learn meaningfull high-level semantic features that are shared between instances of the same class, while SSL might capture irrelevant low level visual features (e.g., related to instance background). Thus high ImageNet performance guarantees that the features learnt are semantically meaningful and SSL learns diverse features.
This observation is supported by recent work that combine both supervised and self-supervised losses to improve transferability \cite{khosla2020supervised,islam2021broad}, yet those require intervention self-supervision stage and the transferability is attributed to other less important factors than feature diversity such as Centered Kernel Alignment (CKA)~\cite{kornblith2019similarity} and intra-class variations.

Our contribution in this work is twofold; We first introduce \textit{Feature Diversity} as a metric for assessing a model's transferability to replace the standard Imagenet Score, and secondly introduce a simple and generic method-agnostic approach, \textit{Controlled Label Injection (CIS)}, for integrating supervised and self-supervised training. 
We empirically observe that:
\begin{align}
\textit{CIS} = \text{Imagenet Accuracy} \times \text{Feature Diversity}
\end{align}
highly correlates with trasferability, as shown in Figure~\ref{fig:tl_correlation}, and thus provides a correction to the Imagenet accuracy as a better predictor of transferability.

Our propose training method \textit{Controlled Label Injection}, enables injecting label information into any self-supervised pre-trained model in a controlled manner, for generating models of different feature diversity and Imagenet accuracy. The resulting models increase ImageNet performance while either improving or maintaining feature diversity of the self-supervised model.
We show that this leads to higher transferability.

We validate our approach over both CNNs (ResNets~\cite{he2016deep}) and vision transformers (ViT~\cite{dosovitskiy2021an}), several self-supervised pre-training methods (e.g., MoCo-v2~\cite{chen2020improved},
% SimCLR~\cite{chen2020simple},
SwAV~\cite{caron2020unsupervised} and MAE~\cite{MaskedAutoencoders2021}), several formulations of feature diversity, several downstream vision tasks, including multi-label classification on the MS-COCO~\cite{lin2014microsoft} dataset and a variety of 14 single-label classification datasets.

The following paper layout: In section~\ref{sec:feature_diversity} we introduce the notion of feature diversity.  In section~\ref{sec:LabelInjection} we the describe the \textit{Controlled Label Injection} scheme, for generating models of different feature diversity and Imagenet accuracy.
In section~\ref{sec:exp} we describe the experimental setup, downstream tasks and datasets, alternative transferability metrics.
In section \ref{sec:fesature_importance} we utilize the \textit{Controlled Label Injection} scheme for improving the transferability of pretrained models, by increasing their \textit{Calibrated Imagenet Score}, either by maintaining feature diversity while improving Imagenet accuracy or increasing both.  We show in that feature diversity is more important for transferability than other previously suggested factors~\cite{kornblith2021better,islam2021broad}, such as the level of abstraction learnt by the model and class separation.
We measure the diversity of the learned features and empirically confirm that feature diversity plays an important role, together with ImagenNet performance, in the transferability of the pre-trained model.

\begin{figure}[htb]
\centering
\begin{subfigure}{.49\textwidth}
  \centering
    \includegraphics[width=0.98\textwidth, height=!]{figures/tl_vs_imgnt.png}
  \label{fig:label_injection_cka}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
    \includegraphics[width=0.98\textwidth, height=!]{figures/tl_vs_calibarated.png}
  \label{fig:label_injection_calibrated}
\end{subfigure}
\caption{Transferability vs Imagent accuracy (Left) and the Calibrated Imagenet Score (Right). The Calibrated Imagenet Score correlates with transferability significantly better.}
\label{fig:tl_correlation}
\end{figure}

==> intro_old.tex <==
\section{Introduction}
\textcolor{red}{convolutional neural networks (CNNs) \cite{krizhevsky2012imagenet,lecun1989backpropagation} revolutionized computer vision arguably due to the discovery that feature representations learned on a pre-training task can transfer useful information to target tasks \cite{girshick2014rich,donahue2014decaf,zeiler2014visualizing}. In recent years, a well-established paradigm has been to pre-train models using large-scale supervised data (e.g., ImageNet~\cite{russakovsky2015imagenet}) and then to fine-tune the models on target tasks that often have less training data \cite{tan2018survey}. Pre-training has advanced the state-of-the-art on many tasks, including action recognition \cite{simonyan2014two,carreira2017quo}, object detection \cite{girshick2014rich,ren2015faster} and semantic segmentation \cite{long2015fully,he2017mask}.}


The success of Deep Neural Networks (DNNS) in a variety of computer vision tasks is largely related to their ability to transfer feature representations learned on a pre-trained task to leverage others.
A common practice is to pre-train a model on a large-scale supervised dataset such as ImageNet~\cite{russakovsky2015imagenet} and fine-tune it on the downstream (target) dataset that is typically of a smaller scale.
This practice has advanced the state-of-the-art in tasks such as image classification~\cite{liu2021query2label,ridnik2021ml}, object detection~\cite{liu2021swin,ren2015faster} and semantic segmentation~\cite{he2017mask,liu2021swin}.

The pursuit after better pretrained models coincided with pushing the state-of-the-art performance on ImageNet, as it was systematically shown that supervised pre-trained models that perform better on ImageNet also tend to perform better when fine-tuned on other vision tasks \cite{kornblith2019better}.

However, recent works demonstrate that self-supervised pre-training without any label information can also learn effective representations from upstream data (e.g., ImageNet) and even surpass supervised methods when transferring to downstream tasks, although their performance on ImageNet is significantly worse \cite{chen2020simple,he2020momentum,grill2020bootstrap,chen2021exploring,zbontar2021barlow,ericsson2021well}. 
This calls for identifying the additional factors, on top of Imagenet accuracy, that make models transferable.



Motivated by the success of self-supervised pre-training, we identify the key differences from the supervised counterpart. Unlike the latter, that focuses on class-level discrimination, the former is mainly based on instance discrimination, where models are trained to keep variants of the same instance close together in the representation space, and sometimes also, separated from different instances. Thus the self-supervised approach effectively captures richer and more diverse and discriminative features of varying levels of abstraction, that are useful for many downstream tasks, compared to more high level class-discriminative features learned by supervised methods. With this understanding, we propose to consider feature diversity as a key objective. We measure the diversity of the learned features and empirically confirm that feature diversity plays an important role, together with ImagenNet performance, in the transferability of the pre-trained model.

However, diversity cannot stand by its own, considering that a random model obviously has high feature diversity yet very poor transferability. Thus high ImageNet performance guarantees that the features learnt are also meaningful. Furthermore, without any supervision, self-supervised models are prone to ignore transferable high-level semantic features that are common to a class of instances, and may capture detailed but irrelevant low level visual features (e.g., related to instance background).
% downstream tasks, e.g. fine-grained classification (Islam et al., 2021).
This observation is supported by recent work that combine both supervised and self-supervised losses to improve transferability \cite{khosla2020supervised,islam2021broad}, yet those require to intervene in the very self-supervision stage and the transferability is attributed to other less important factors than feature diversity (e.g., Centered Kernel Alignment (CKA)~\cite{kornblith2019similarity} and intra-class variations). 

In this work we highlight the importance of feature diversity and introduce a simple and generic method-agnostic approach, for integrating supervised and self-supervised training. More specifically, our method enables injecting label information into any self-supervised pre-trained model in a controlled manner, and through that increases ImageNet performance while at the same time either improving or maintaining feature diversity of the self-supervised model. We show that this leads to higher transferability. 

We validate our approach over both CNNs (ResNets~\cite{he2016deep}) and vision transformers (ViT~\cite{dosovitskiy2021an}), several self-supervised pre-training methods (e.g., MoCo-v2~\cite{chen2020improved},
% SimCLR~\cite{chen2020simple},
SwAV~\cite{caron2020unsupervised} and MAE~\cite{MaskedAutoencoders2021}), several formulations of feature diversity, several downstream vision tasks, including multi-label classification on the MS-COCO~\cite{lin2014microsoft} dataset and a variety of 14 single-label classification datasets.

==> method.tex <==
\section{Method}
\subsection{Motivation}
\begin{itemize}
    \item Self-supervided learning (SSL) provides better pretrained models from their fully supervised counterparts.
    \item The underlying contrastive learning views each sample as a unique class. Hence, we expect features learnt by SSL to be richer and more diverse compared to the supervised models of much smaller set of classes.
    \item Once should still consider leveraging the human knowledge acquired in the labeling process.
    \item To this end, we propose a simple way to control the label information injected to the diverse SSL backbone model while maintaining its feature diversity.
\end{itemize}


